Hidden Structures of Black Holes

This thesis investigates two main topics concerning black holes in extensions of general relativity inspired by string theory. First, the structure of the equations of motion underlying black hole solutions is considered, in theories of D-dimensional gravity coupled to scalars and vectors. For solutions preserving supersymmetry, the equations of motion have a dramatic simplification: they become first-order instead of the second-order equations one would expect. Recently, it was found that this is a feature some non-supersymmetric black hole solutions exhibit as well. We investigate if this holds more generally, by examining what the conditions are to have first-order equations for the scalar fields of non-supersymmetric black holes, that mimic the form of their supersymmetric counterparts. This is illustrated in examples. Second, the structure of black holes themselves is investigated. String theory has been successful in explaining the Bekenstein-Hawking entropy for (mainly supersymmetric) black holes from a microscopic perspective. However, it is not fully established what the interpretation of the corresponding 'microstates' should be in the gravitational description where the black hole picture is valid. There have been recent advances to understand the nature of black hole microstates in the gravity regime, such as the fuzzball proposal. A related idea says that black hole configurations with multiple centers are related to microstates of single-centered black holes. We report on work relating both pictures. As an aside, a relation between violations of causality for certain spacetimes (presence of closed timelike curves in the geometry) and a breakdown of unitarity in the dual conformal field theory is given.

==> App_Ndl.tex <==
\selectlanguage{dutch}
\chapter{%\chaptertypeset 
Nederlandse samenvatting}\label{app:NDL}

\ponslijn{Dit doctoraatswerk behandelt zwarte gaten binnen de theoretische natuurkunde. Het doel van deze appendix is een kort overzicht te geven van de achtergrond van dit verslag, voor lezers zonder technische kennis van de natuurkunde. We beginnen met een duiding van wat een zwart gat is en waarom zwarte gaten interessante studie-objecten vormen (sectie \ref{s:NDL-1}). Dan volgt een korte beschrijving van de ruimere context van dit doctoraatswerk (de tak van de theoretische natuurkunde die onder de naam snaartheorie valt) in sectie \ref{s:NDL-2} en een overzicht van twee grote onderzoekstakken van de snaartheorie die aan bod komen in de verschillende hoofdstukken van dit proefwerk, in sectie \ref{s:NDL-3}. In sectie \ref{s:NDL-4} tenslotte komt (beknopt) het origineel onderzoek van dit doctoraat aan bod.}


\section{Hoe en waarom van zwarte gaten}\label{s:NDL-1}
Deze thesis is het verslag van onderzoek rond zwarte gaten. Een zwart gat is een object waarvoor de aantrekking door de zwaartekracht zo groot is dat niets, zelfs niet het licht, eraan kan ontsnappen. We gaan daarom eerst dieper in op de zwaartekracht.


\subsubsection{De natuur modelleren: zwaartekracht en haar limitaties}
In de natuurkunde (en bij uitbreiding in alle wetenschappen) gebruiken we modellen om fenomenen rondom ons te verklaren. Zo weten we dat de beweging van voor\-wer\-pen zoals vallende regendruppels, stenen die je wegwerpt, rijdende auto's, noem maar op, beschreven kan worden door allerlei krachten die op die voorwerpen inwerken en beweging veroorzaken. (Denk aan de kracht die je moet uitoefenen om een steen weg te gooien.) Er is \'e\'en kracht die zich onderscheidt van alle andere: de zwaartekracht. Dit is de kracht die ervoor verantwoordelijk is dat we met onze voeten op de grond blijven en niet wegzweven, de kracht die ervoor zorgt dat regendruppels naar de aardbodem toe vallen. Maar ze is ook verantwoordelijk voor de beweging van planeten rond de zon, de beweging van sterren in het heelal.  

De zwaartekracht is uniek omdat ze de enige kracht is die werkt tussen elke twee voorwerpen die je je maar kan indenken. Hoewel ze alomtegenwoordig is, hebben we haar nog steeds niet volledig begrepen: tot op vandaag vormt ze een enorme theoretische uitdaging. Eind zeventiende eeuw zette Newton een enorme stap  door een zeer goede beschrijving van de zwaartekracht op te stellen die de beweging van vallende voorwerpen verklaart hier op aarde, maar evengoed de planetenbeweging rond de zon uitlegt. Een dikke tweehonderd jaar later stelde Einstein de zwaar\-te\-krachts\-theo\-rie op punt met zijn algemene relativiteitstheorie, die een goede verklaring biedt van de zwaartekracht op astronomische schalen. Zo verklaart de theorie bijvoorbeeld met succes de geobserveerde uitdijing van het heelal en verklaart ze waargenomen correcties op de vorm van planeetbanen t.o.v.\ Newtons theorie.\footnote{I.h.b.\ gaat het om de precessie van het perihelium voor (bijna-)ellipsbanen. Voor de planeet Mercurius is dit effect meetbaar en komt de observatie overeen met de voorspelling uit relativiteit. } De gravitatietheorie faalt echter op kleine schaal. Op (sub-)microscopische schaal is de materie opgebouwd uit moleculen, die dan weer bestaan uit atomen; elk atoom is op zijn beurt samengesteld uit de kleinst waargenomen stukjes materie: elementaire deeltjes. Het begrijpen van de interacties tussen die elementaire deeltjes is van groot belang om te weten hoe materie in elkaar zit. Voorlopig hebben we een goed zicht op alle krachten tussen die elementaire deeltjes,\footnote{Die krachten zijn terug te brengen tot twee fundamentele interacties (de elektrozwakke interactie  -- beschrijft electromagnetisme en de zwakke kernkracht -- en de  sterke interactie).} behalve de zwaartekracht. De beschrijving van de krachten tussen elementaire deeltjes op kleine schaal gebeurt volgens de principes van wat we kwantummechanica noemen. De manier waarop we kwantummechanica beschrijven werkt echter niet voor de zwaartekracht. We hebben dus een probleem:

\outlook{PROBLEEM:}{We begrijpen de zwaartekracht op grote schaal, maar op niveau van de allerkleinste elementaire deeltjes loopt het mis.
%Op grote schaal weten we dat de zwaartekracht werkzaam is tussen alle materie. Op kleine schaal zou dit ook zo moeten zijn, maar we weten niet hoe de elementaire deeltjes be\diaeresis{i}nvloed worden door de zwaartekracht. We zeggen dat we \textit{geen goede kwantum-gravitatie} theorie hebben.
}

We kunnen op verschillende manieren de tekortkomingen van de zwaartekracht zien. E\'en ervan is door de zwaartekracht te bestuderen waar ze op haar sterkst is: in zwarte gaten. 


\subsubsection{Zwarte gaten}
 %Eerst: zwaartekracht $\to$ gravitatie. Dan``: algemene relativiteitstheorie. 
Een zwart gat  is een deel van de ruimte waaruit niets of niemand kan ontsnappen, zelfs het licht niet. Van buitenaf gezien ziet het er dus volledig zwart uit, wat meteen de naam verklaart. Het bestaan van een zwart gat wordt voorspeld door Einsteins gravitatietheorie: wanneer zulke grote concentraties massa in een bepaald volume wordt gestopt, dat niets nog aan de zwaartekracht ervan kan ontsnappen, ontstaat een zwart gat. We kunnen een zwart gat zien als iets waar we vanalles kunnen ingooien, maar waar niets terug uit kan komen. In de natuur worden zwarte gaten gevormd wanneer zeer massieve sterren instorten onder invloed van hun eigen gewicht. Zo bevindt er zich bijvoorbeeld een gigantisch zwart gat in het centrum van ons melkwegstelstel.\footnote{Tevens ontdekte men zwarte gaten in de centra van vele andere melkwegstelsels.}
%dat volume kan wegspringen. In het bijzonder wordt zelfs het licht, de snelste aller boodschappers, door een zwart gat gevangen. Van buitenaf gezien ziet die massaconcentratie er dus volledig zwart uit, wat meteen de naam van het ding verklaart.

%\comment{Hoe onstaan ze? Evolutie naar singulariteit. Waar komen ze voor?}

%Laten we beginnen met een intuitieve voorstelling.  Beeld je in dat je een steen omhoog gooit. Die steen zal even de lucht doorklieven, maar zal dan terug vallen op de grond. Dit komt niet zomaar, er is een aantrekking tussen de steen en de aarde die hier verantwoordelijk voor is: de zwaartekracht. De zwaartekracht van de aarde is echter niet oneindig sterk: als we hard genoeg zouden kunnen gooien, zouden we de steen de ruimte in kunnen gooien om nooit meer weer te keren. De snelheid die nodig voor een steen die je gooit is om aan de zwaartekracht van aarde te ontsnappen, is ongeveer $40\,000$ kilometer per seconde.  We noemen dit de ontsnapingssnelheid van de aarde. We kunnen op een gelijkaardige manier een ontsnappingssnelheid defini\"eren voor andere hemellichamen: die van de maan is ongeveer zes maal kleiner dan die van de aarde, omdat de maan zes maal minder massa heeft. De ontsnappingssnelheid van de zon is dan weer vele malen groter, omdat de zon veel meer massa heeft dan onze aardbol. Wanneer een hemellichaam (een ster bv.) zo veel massa heeft in een bepaald volume dat de ontsnappingssnelheid groter wordt dan de snelheid van het licht, zitten we met een probleem. We weten dat niets zich sneller dan het licht kan verplaatsen, dus dit zou betekenen dat geen enkele steen, hoe hard we ze ook gooien nog van die massieve ster kan ontsnappen. Sterker nog: stel dat we met een zaklamp omhoog zouden schijnen vanop het oppervlak van die ster. De lichtstralen zouden ook niet meer kunnen ontsnappen. We kunnen bezwaarlijk nog van een ster spreken

%We moeten bij het bovenstaande beeld wel een kanttekening plaatsen. Wanneer de zwaartekracht van een object erg groot wordt, moeten we eigenlijk ons kader bijstellen. De `gewone' zwaartekrachtswet die terecht op middelbare scholen onderwezen wordt (`de zwaartekrachtswet van Newton') kan zeer nauwkeurig alledaagse fenomenen bescrijven (een vallende appel), maar slaagt er niet in om op astronomische schalen juiste voorspellingen te doen. Hiervoor is de algemene relativiteitstheorie nodig, zoals ze werd naar voren geschoven door Einstein. Volgens de algemene relativiteitstheorie heeft de aanwezigheid van materie, van massa, een impact op de ruimte en de tijd: in de nabijheid van massieve objecten worden ruimte en tijd gekromd. Dit lijkt misschien erg raar, maar de gevolgen van de algemene relativiteitstheorie zijn wel degelijk bevestigd. 

%Zo zijn mensen er al in geslaagd om sterren te zien die zich achter de zon bevinden: rond de zon, een massieve ster, worden de lichtstralen van de achterliggende sterren afgebogen, wat ons toelaat om toch te zien wat er zich achter bevindt (we noemen dit een gravitatielens). Andere punten waar de theorie erg succesvol bleek is in het voorspellen van kleine correctie op de banen van de planeten rond de zon. 
%\comment{Slechts een van vele voorspellingen...} Verder hebben mensen kunnen waarnemen dat het heelal uitdijt. Deze uitdijing wordt verklaard binnen de algemene relativiteitstheorie: het heelal zou ge\"evolueerd zijn uit \'e\'en punt, waarna het is blivjen uitzetten tot de gigantische omvang die het nu heeft. Dit wordt ook wel eens `de Oerknal' genoemd. Er zijn nog veel andere succesverhalen verbonden aan de algemene relativiteitstheorie, maar die laten we voor wat ze zijn. We gaan verder met het studie-onderwerp van deze thesis: zwarte gaten. We weten dat massa de ruimte kromt. Wanneer we meer en meer massa in een gegeven volume stoppen, wordt de ruimte errond meer en meer gekromd. Als we blijven doorgaan, zal de massa-concentratie zo groot worden dat lichtstralen, de snelste boodschappers die er bestaan, zo sterk worden afgebogen dat ze niet meer kunnen ontsnappen.\comment{Hernieuwing: zwart gat}

In een eerste poging om zwarte gaten op microscopische schaal te beschrijven (via een beschrijving binnen kwantummechanica), toonde Stephen Hawking in de jaren 1970 aan dat zwarte gaten een temperatuur hebben en thermische straling uitzenden: ze zijn dus toch niet zo zwart als op het eerste zicht gedacht wordt. De thermische straling is te vergelijken met  die van hete kolen in een open haard. Afhankelijk van de temperatuur, geven de kolen meer of minder warmtestraling af, of zelfs zichtbare straling als ze goed heet zijn (denk aan roodgloeiende kolen, die rood licht uitzenden). Hawking berekende een gelijkaardig effect voor zwarte gaten.\footnote{Let wel: de temperatuur van de zwarte gaten in het heelal is bijzonder klein. De temperatuur is omgekeerd evenredig met de massa van een zwart gat: hoe massiever, hoe lager de temperatuur. Voor een zwart gat met dezelfde massa als die van de zon, ligt de temperatuur rond de $-273^\circ$ Celsius!} Een gevolg van de thermische eigenschappen, is dat een zwart gat een bepaalde hoeveelheid van wat we in de natuurkunde \textit{entropie} noemen bezit. De entropie is een maat voor het gebrek aan informatie dat we over een systeem hebben, in dit geval duidt het op het gebrek aan informatie over waaruit het zwarte gat bestaat. Typisch duidt de hoeveelheid entropie van een systeem erop,  op hoeveel manieren we het systeem microscopisch kunnen realiseren. Om het concept van entropie (dat een centraal onderdeel vormt van dit doctoraat) te verduidelijken, even een analogie. Beeld je in dat iemand een grote hoop ballen heeft in drie kleuren: rode, gele en blauwe. Hij kiest er willekeurig een uit en stopt die bal in een zwarte doos. Wanneer die persoon jou die doos geeft, kan je hoogstens concluderen dat er \'e\'en bal in de doos zit. Zonder in de doos te kijken, kan je echter niet weten welke kleur de bal heeft. Er zijn drie mogelijkheden (blauw, rood of geel). We zouden kunnen zeggen dat het getal `3' een maat is voor  `het gebrek aan informatie' over wat er in de doos zit (de entropie). 
%Wanneer er twee ballen in de doos zouden zitten, zouden er 6 kleurcombinaties mogelijk zijn (blauw-blauw, rood-rood, geel-geel, geel-rood, geel-blauw en rood-blauw): een doos met twee ballen heeft entropie `6'. Als we zo doorgaan, kunnen we aan elk aantal ballen dat in de doos zit een entropie associ\"eren. 
%Het aantal ballen is een `macroscopische parameter' en 
De entropie geeft een idee over het aantal `microscopische toestanden' dat met de zwarte doos overeenkomt. 
%In een meer realistisch voorbeeld, zouden we een glaasje water kunnen nemen. Op microscopische schaal zijn er ongelooflijk veel manieren waarop de moleculen van het glas water zich zouden kunnen organiseren. We zeggen dat het glaasje water een welbepaalde entropie heeft. 
Op een gelijkaardige manier heeft een zwart gat ook een bepaalde hoeveelheid entropie. 
%De entropie van een zwart gat wordt groter als het zwart gat meer massa heeft, wat ergens ook logisch is: hoe groter de ruimte die een zwart gat verbergt, hoe meer informatie het zwart gat van ons verbergt.\footnote{Deze analogie loopt een beetje mankt. Ze suggereert misschien dat de entropie van een zwart gat evenredig is met het volume van de ruimte verborgen achter de waarnemingshorizon. Dit is niet juist, verrassend genoeg blijkt dat de entropie evenredig is met de oppervlakte van de waarnemingshorizon.}

%De identificatie van een zwart gat als een object met temperatuur en entropie, dat straling uitzendt roept vragen op 
Het bovenstaande plaatje roept een aantal vragen op die de algemene relativiteitstheorie niet kan beantwoorden. Bijvoorbeeld, als een zwart gat een entropie heeft, wat zijn dan de microstoestanden die ermee overeenkomen? In het voorbeeldje van de zwarte doos met een bal erin, weten we perfect welke die mogelijke microtoestanden zijn (gele bal, rode bal of blauwe bal). 
%In een meer realistisch voorbeeld zouden we twee identieke glazen kunnen gevuld met water op kamertemperatuur. 
%Ook voor het glaasje water hebben we een microscopische verklaring voor de entropie: elke microtoestand is een bepaalde schikking van de moleculen op microscopische schaal. 
% Een microscopische verklaring van de entropie voor zwarte gaten is echter niet voorhanden, omdat er binnen Einsteins algemene relativiteitstheorie geen beschrijving is van microscopische toestanden voor een zwart gat. We hebben dus wel een entropie, die duidt op een groot aantal microtoestanden, maar we weten helemaal niet wat die toestanden zouden kunnen zijn. Ten tweede zijn er ook problemen die opduiken als we de warmtestraling van een zwart gat ter harte nemen. Langs de ene kant weten we dat volgens de principes van de kwantummechanica de hoeveelheid informatie behouden blijven, of anders gezegd, een bepaalde eindtoestand van een proces moet terug te traceren zijn naar zijn begintoestand. Langs de andere kant, is de  thermische straling die uit het zwart gat komt, enkel bepaald door de temperatuur en de massa van het zwart gat. Dramatisch gezegd: stel dat we een persoon van 70 kg in het zwart gat gooien, of een zak cement van 70 kg, de straling die vervolgens uit het zwart gat komt is in beide gevallen hetzelfde. De informatie die we kunnen associ\"eren met wat we erin hebben gegooid (een persoon,  een zak cement) is volledig verdwenen.  Dit probleem met de wetten van de kwantummechanica wordt ook wel de \textit{informatieparadox} genoemd. En ten derde is er nog een probleem dat we niet bespraken. Een ster die ineenstort en een zwart gat vormt, zal volgens Einsteins gravitatietheorie uiteindelijk onder invloed van zijn eigen zwaartekracht  volledig ineenkrimpen tot \'e\'en punt. In dit punt is de materie van de invallende ster oneindig dicht samengepakt, we spreken van een \textit{singulariteit}. In de aanwezigheid van die singulariteit met oneindige dichtheid kan de algemene relativiteitstheorie geen goede beschrijving meer bieden.\footnote{Iets technischer: de aanwezigheid van een punt met oneindige massadichtheid leidt tot een oneindig sterke kromming van de ruimte-tijd en de concepten `tijd' en `ruimte' zijn niet meer goed gedefinieerd binnen de algeme relativiteitstheorie}



\outlook{Problemen oplossen?}{We zien dat zwarte gaten duiden op onvolledigheden in Einsteins theorie van de zwaartekracht. Een goede theorie van gravitatie, die werkt op alle schalen (van het allerkleinste tot het allergrootste), moet deze problemen kunnen oplossen. Zo een theorie zou de zwaartekracht verenigen met de wetten van de kwantummechanica. We noemen ze dan ook een kwantumgravitatie-theorie. Voorlopig is de snaartheorie de meest veelbelovende kandidaat voor een dergelijke kwantumgravitatie-theorie. Daarom is het van groot belang om te kijken of de snaartheorie een antwoord biedt op bovenstaande problemen.}

%de kwantummechanica: Hawkings berekeningen steunden al op enkele aspecten van kwantummechanica. Een goede theorie die kwantummechanica en algemene relativiteit verzoent, moet ook het probleem van de singulariteit doen verdwijnen: voordat de singulariteit zou gevormd, zouden kwantummechanische effecten op microscopischie schaal het moeten overnemen en men verwacht dat in kwantum gravitatie zwarte gaten geen singulariteit meer hebben.


\section{Kan snaartheorie zwarte gaten verklaren?}\label{s:NDL-2}

\subsubsection{Snaartheorie}
%Wanneer we zouden inzoomen op een stukje materiaal, zouden we zien dat het bestaat uit moleculen. Moleculen zijn dan weer opgebouwd uit atomen. Elk atoom kan je dan weer zien als een samenhangsel van nog kleinere deeltjes, zoals bv. electronen. 
We hebben eerder gezien dat -- voor zover we weten -- materie op kleine schaal bestaat uit een aantal elementaire deeltjes. Die elementaire deeltjes zijn de kleinste bouwstenen van materie die tot nu toe zijn waargenomen. Voor zover we hebben kunnen zien in experimenten, bijvoorbeeld ~in grote deeltjesversnellers zoals die in het CERN in Gen\`eve, zien ze eruit als puntjes die zich bewegen in de ruimte.  De \textit{snaartheorie} komt met een radicaal ander voorstel: elementaire deeltjes zijn helemaal geen puntjes volgens deze theorie, maar hele kleine snaartjes. Zoals de snaar van een gitaar verschillende tonen kan produceren, zo kan het kleine snaartje, afhankelijk van hoe het trilt, zich manifesteren als een ander elementair deeltje. De lengte van de snaartje is echter zo klein, dat de snaartjes er voor ons, waarnemers, uitzien als puntdeeltjes. Het mooie van de snaartheorie is dat ze op een natuurlijke wijze  kwantummechanica en gravitatie in \'e\'en omvattende beschrijving giet. Dit komt omdat ze de beschrijving op al\-ler\-klein\-ste schaal van materie (elementaire deeltjes en hun interacties) verklaart volgens de principes van de kwantummechanica \'en omdat trillende snaren ook een deeltje kunnen beschrijven dat verantwoordelijk is voor de zwaartekracht (het zwaartekrachtsdeeltje of graviton). Op die manier hebben we een kwantumgravitatie-theorie, een beschrijving van de zwaartekracht  op kleinste schaal.

Er zijn een aantal specifieke eigenschappen die de snaartheorie  kenmerken. De merkwaardigste is misschien wel dat ze voorspelt dat er in plaats van drie dimensies (d.w.z.~drie bewegingsrichtingen: vooruit -- achteruit, onder -- boven, links -- rechts) negen dimensies zouden zijn. Dit lijkt misschien tegenstrijdig (We zien toch maar drie dimensies? Waar zijn die andere zes?) maar we kunnen toch de snaartheorie linken aan onze wereld. De idee die erachter ligt is dat de overige zes dimensies heel klein kunnen zijn, zodat de wereld er effectief uitziet alsof er maar drie dimensies zijn. Jammer genoeg brengt die kleine-extra-dimensie hypothese een probleem met zich mee. Omdat er in de snaartheorie een gigantisch aantal manieren is waarop we de extra zes dimensies klein kunnen maken, betekent dit ook dat er een gigantisch aantal mogelijke beschrijvingen van onze wereld volgt uit de snaartheorie. Om die reden is het moeilijk om uit de snaartheorie informatie te halen over onze natuur. Daar knelt het schoentje: voorlopig heeft snaartheorie nog geen voorspellingen kunnen doen die we kunnen testen in experimenten. Omgekeerd is het ook zeer moeilijk om uit huidige experimenten informatie te halen die ons kan helpen om meer te weten te komen over de snaartheorie. De huidige deeltjesversnellers geven ons bijvoorbeeld zeer nuttige informatie over de subatomische opbouw van de materie, maar we kunnen nog steeds niet `fijn' genoeg kijken om te zien of een elementair deeltje een echt puntje, dan wel een snaartje is. Behoudens gelukkig toeval, is het helemaal niet duidelijk dat we binnen afzienbare tijd (of zelfs ooit) afdoende experimenteel bewijs zullen hebben voor de snaartheorie.
%Reden daarvoor is bijvoorbeeld dat gigantisch aantal mogelijke beschrijvingen van onze wereld, maar ook de 

Er is dan ook al behoorlijk wat kritiek gekomen op de theorie, vooral binnen de natuurkundige gemeenschap zelf. Moet de ultieme scherprechter voor een natuurkundige niet het experiment zijn? Wat is een theorie waard die we niet kunnen testen in het laboratorium?\footnote{Nuttige waarnemingen buiten het laboratorium mogen ook, natuurlijk} Wel, vooreerst is het niet uitgesloten dat er \textit{aanmoedigingen} te rapen zijn uit toekomstige experimenten. 
%Het is misschien heel moeilijk om uit snaartheorie een antwoord te krijgen op al onze experimentele vragen, maar er zijn zeker aspecten die verdere studie van snaartheorie promoten. 
Zo voorspelt de snaartheorie bijvoorbeeld dat er een veel groter aantal elementaire deeltjes zou bestaan dan tot nu toe waargenomen en dat er bepaalde verbanden tussen die deeltjes zijn die we nog niet ontdekt hebben (we bundelen die verbanden onder de naam `supersymmetrie'). Het is niet uitgesloten dat de LHC-versneller in CERN die momenteel operationeel is, die nieuwe deeltjes ontdekt. Dit zou geen bewijs zijn van snaartheorie, maar zou alleszins een idee geven dat we op goede weg zijn. Langs de andere kant kunnen we ook de idee van precieze voorspellingen even laten voor wat het is en tenminste de snaartheorie uitpluizen op wat we `theoretische volledigheid' zouden kunnen noemen. De studie van zwarte gaten in de snaartheorie zou een voorbeeld kunnen zijn. Als snaartheorie de pijnpunten van zwarte gaten in Einsteins gravitatietheorie kan oplossen (Hoe zit het met die entropie? De informatieparadox? De singulariteit?) zijn we al een eind op weg. Als ze dat niet zou kunnen, heeft de snaartheorie een probleem. In die zin hebben we een theoretische test voor de snaartheorie. Het is dat laatste pad dat we volgen.

\subsubsection{Snaartheorie en zwarte gaten}

%Binnen de snaartheorie is het mogelijk om voor bepaalde zwarte gaten de entropie te verklaren vanuit een microscopisch oogpunt. 
%Om uit te leggen hoe dit in zijn werk gaat, kunnen we het zwart gat zwart gat voorstellen als een zwarte doos, zoals eerder. 
We zouden graag weten waaruit het zwart gat is opgebouwd, wat zijn `microtoestanden' zijn, of in de analogie met de zwarte doos en de gekleurde ballen, welke gekleurde ballen er allemaal in de doos kunnen zitten.
Binnen de snaartheorie probeerde men reeds de microtoestanden van een zwart gat te vinden, via een gedachtenexperiment.  Wat als we ons inbeelden hoe het zwart gat eruit ziet als de zwaartekracht zwakker en zwakker gemaakt wordt? Op een bepaald moment zal de zwaartekracht zo zwak worden dat het zwarte gat terug uiteenvalt in `gewone' materie. In de doos-analogie: de zwarte doos verdwijnt en er blijven ballen over. In de beschrijving waarin de zwaartekracht niet meer aanwezig is, kunnen we dus perfect weten welke soort ballen er allemaal in de doos kunnen zitten, zie figuur \ref{fig:NDL-BH_counting}. Binnen de snaartheorie kunnen we deze analogie exact maken: de `gekleurde ballen' zijn dan welbepaalde microscopische snaartoestanden. Wanneer men het aantal van die microtoestanden telt, dan ziet men  dat dit aantal exact de entropie van het zwart gat reproduceert. We hebben de entropie van een zwart gat kunnen verklaren!\footnote{\ldots toch in de veronderstelling dat we de zwaartekracht mogen minimaliseren. Mijn doc\-to\-raats\-werk concentreert zich op het geval waarin de zwaartekracht wel een rol speelt, zie onder.} Deze berekening stamt uit 1995 en was een enorm succes van de snaartheorie. Dertig jaar al was men vruchteloos op zoek naar een verklaring voor de zwarte-gat entropie.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\centering
\begin{picture}(100,80)
\put(-50,65){\epsfig{figure=DoosBallen.ps,width=.17\textwidth,angle=-90}} 
\put(-20,0){\textit{\textbf{Sterkere zwaartekracht}}}
\end{picture}
\caption[Weak vs.~strong gravity as balls in a box. (Dutch)]{Als de zwaartekracht zwak is, laat snaartheorie ons toe om te zien waaruit het zwart gat is opgebouwd, in analogie met de zwarte doos die gekleurde ballen bevat.}
\label{fig:NDL-BH_counting}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Eerlijksheidshalve moeten we toegeven dat we een beetje vals hebben gespeeld. De vergelijking met een aantal microstoestanden van snaren waarin we doen alsof de zwaartekracht er niet is, werkt enkel voor een speciale klasse van zwarte gaten, die supersymmetrisch worden genoemd. Deze supersymmetrische zwarte gaten zijn bijzonder onrealistisch: ze dragen elektrische ladingen die zo gigantisch groot zijn, dat ze in de natuur nooit gerealiseerd kunnen worden. En met te doen alsof de zwaartekracht er niet is, hebben we nog geen idee gekregen wat nu werkelijk de  microtoestanden zijn van een zwart gat (de \'echte `ballen in de zwarte doos') in het realistische geval dat de zwaartekracht wel een rol speelt. 

Met andere woorden hebben we deels een antwoord op het entropievraagstuk, maar er blijven (minstens) twee vragen over, te beantwoorden in een regime waar de zwaartekracht niet verwaarloosd wordt:
\begin{itemize}
\item[\ra] Wat is de \textit{microscopische structuur} van een zwart gat?
\item[\ra] Wat weten we van meer realistische, \textit{niet-supersymmetrische} zwarte gaten?
\end{itemize}
%De eerste van deze twee vragen zou hopelijk ook een antwoord kunnen bieden op de informatieparadox en de problemen met de singulariteit: als we weten wat een eigenlijke microtoestand van een zwart gat is,
De twee bovenstaande vragen vormden de basis voor de twee onderzoeksgebieden waarbinnen dit doctoraatswerk valt.  We zullen er nu dieper op ingaan.

\section{Twee onderzoeksgebieden}\label{s:NDL-3}
%In het licht van de vragen die hierboven geopperd zijn, kunnen we ingaan op hoe die vragen aangepakt werden en worden binnen de context van de snaartheorie. 
%Nu volgt een korte shets van de achtergrond van de twee onderzoeksgebieden waarin ik actief bijdroeg in dit doctoraatswerk.\comment{Leg SUGRA uit? Regime waarin we puntdeeltjes bekijken en gravitatie met een hoop extra deeltjes.}

\subsubsection{Microscopische structuur van een zwart gat: de pluisbal}

%We zagen voordien dat in het klassieke beeld zoals voorspeld door Einsteins gravitatie, een zwart gat een punt is van oneindige dichtheid, een \textit{singulariteit}, omgeven door een waarnemingshorizon.  De ruimte tussen de singulariteit en de waarnemingshorizon is letterlijk leeg in dit model: alles wat binnen de waarnemingshorizon terechtkomt kan er niet meer uit en verdwijnt in de singulariteit.

%We hebben ook gezien dat dit leidt tot de \textit{informatieparadox}: van om het even welke combinatie van materie met een bepaalde masse we een zwart gat maken (planeten, sterren, protonen, mensen, zakken cement\ldots), het maakt niet uit. De eindtoestand is altijd datzelfde zwart gat. Dit schendt een basisprincipe binnen de kwantummechanica van irreversibiliteit: we zouden in staat moeten zijn om het eindpunt van een proces terug te brengen tot de begintoestand waaruit het evolueerde, ook voor een zwart gat. Maar als al die toestanden \'e\'en eindpunt hebben,  dan kunnen we het zwart gat niet terugbrengen tot een unieke begintoestand: alle informatie over de materie die het zwarte gat maakte is verloren.

%Zonder een zicht op de microscopische structuur van een zwart gat, hebben we geen oplossing voor belangrijke problemen ainformatieparadox, noch voor de vra
Begin de jaren 2000, kwamen Mathur en zijn medewerkers met een zeer merk\-waar\-dig voorstel omtrent de microscopische structuur van een zwart gat. Volgens Mathur moeten we een zwart gat niet voorstellen als een singulariteit, omringd door lege ruimte, afgescheiden door een waarnemingshorizon, maar door een verdeling van materie in een volume ter grootte van de waarnemingshorizon. De materie binnenin wordt beschreven door de snaartjes van snaartheorie. Hoewel de fundamentele snaartjes zeer klein zijn, kunnen ze - wanneer ze in grote getale aanwezig zijn - samen lange snaren vormen die erg ver kunnen uitstrekken en zo een bal van snaren kunnen vormen ter grootte van een zwart gat. We noemen zo een toestand een `pluisbal',\footnote{De Engelse term die Mathur zelf hanteert is \textit{fuzzball}.} omdat de rand van de bal niet perfect omlijnd is maar een `pluizige' structuur heeft. Het bestaan van de pluisbal volgt uit de \textit{kwantummechanische natuur} van snaartheorie.

Het pluisbal-idee was naar voren geschoven om de problemen die zwarte gaten met zich mee brengen op te lossen. Zo verdwijnt de nare   singulariteit: het binnenste van een zwart gat is niet leeg met een singulariteit erin, maar een ingewikkelde toestand van snaren. Ook de informatieparadox wordt vermeden. De materie die het zwart gat vormt is binnen de snaartheorie zelf een toestand van snaartjes, die aanleiding geeft tot \'e\'en bepaalde pluisbal. We kunnen perfect de toestand van het zwarte gat (de pluisbal) terug linken aan de materie die het zwart gat gevormd heeft. Tenslotte kunnen we het rijtje sluiten door de entropie te begrijpen. Voor iemand die zich ver buiten de pluisbal bevindt, lijkt het nog steeds om een zwart gat te gaan. Pas wanneer we nader zouden gaan kijken, zien we dat de pluisbal de correcte microscopische interpretatie van het zwart gat is. Vergelijk het met twee glazen water die op tafel staan. Als we de inhoud van de twee glazen vergelijken, zien ze er net eender uit. Maar wanneer we zouden inzoomen op de inhoud van elk glas afzonderlijk, dan zien we dat de miscroscopische verdeling van watermoleculen in beide gevallen zeer verschillend is. Op eenzelfde manier moeten we de pluisbal zien als de correcte microscopische beschrijving van een zwart gat. Er zijn echter enorm veel pluisballen die van buitenaf hetzelfde zwart gat lijken te zijn, net zoals er heel veel microscopische configuraties zijn van watermoleculen die van buitenaf het zelfde glaasje water lijken te beschrijven. En net zoals het aantal mogelijke configuraties van watermoleculen de entropie geeft voor het glaasje water, zo kan ook het aantal mogelijke pluisballen de entropie van een zwart gat verklaren. 


%\comment{Binnen GR niet mogelijk. Snaartheorie hiervoor nodig. Lost singulariteit en informatieparadox op. Bv. snaar met lage spanning, can zich uitstrekken tot over grote ruimte. Noot: ook hier weer enkel voor supersymmetrische oplossingen.}

\outlook{Voor dit doctoraat:}{De pluisbal-beschrijving heeft het meeste succes gekend voor de super\-sym\-met\-rische zwarte gaten waarvan eerder sprake. Bovendien veronderstelt de pluisbal-theorie dat er naast de drie uitgestrekte ruimtelijke dimensies die we kennen, een vierde grote dimensie is.\footnote{Vanuit snaartheorie betekent dit dat we slechts vijf extra dimensies klein moeten maken.} Een eerste deel van het onderzoek in deze thesis probeert deze microscopische pluisbal toestanden te begrijpen in het realistische geval van drie (grote) ruimtelijke dimensies zijn. }


\subsubsection{Beschrijving van niet-supersymmetrische zwarte gaten}
%In dit deel van het onderzoek zal ik de niet-fysicus een beetje moeten teleurstellen, omdat een juiste formulering snel technisch wordt. Laat ik een poging doen.
Voor niet-su\-per\-sym\-met\-ri\-sche zwarte gaten is het erg moeilijk om via de snaartheorie de entropie te verklaren, of microtoestanden te vinden. Meer studie is aangewezen. Als eerste stap is het belangrijk om zulke zwarte gaten te onderzoeken in de limiet van snaartheorie waarin de snaren zich gedragen als puntdeeltjes, die bewegen onder invloed van onder andere de gravitatiekracht. In die limiet vinden we uitbreidingen van de algemene relativiteitstheorie met een hoop extra deeltjes die ge\"{\i}nspireerd zijn door de snaartheorie. Die verschillende uitbreidingen van Einsteins gravitatietheorie krijgen de naam supergravitatie mee. 
%
%Het is in de context van supergravitatie dat er momenteel veel onderzoek is naar supersymmetrische en meer realistische niet-supersymmetrische zwarte gaten. 

\outlook{Voor dit doctoraat:}{De wiskundige eigenschappen van niet-supersymmetrische zwarte gaten in supergravitatie worden onderzocht. Op die manier krijgen we geen inzicht in de microscopische `kwantummechanische' natuur van zwarte gaten (omdat we het effect van de kleine snaartjes hebben uitgewist), maar wel een idee van de globale eigenschappen die zwarte gaten hebben (bijvoorbeeld hun temperatuur en de waarde van de entropie). }

\section{Overzicht van de thesis}\label{s:NDL-4}
Nu gaan we in op het originele onderzoek van dit doctoraat (alles hierboven, behoort tot de literatuur), via een overzicht van de hoofdstukken in deze thesis. Het \textit{eerste hoofdstuk} is een algemene introductie, die ruwweg dezelfde onderwerpen bevat als wat in deze Nederlandse samenvatting beschreven is. De idee\"en (zwarte gaten, snaartheorie, verschillende onderzoeksgebieden) worden in technischere taal uitgelegd. Daarna volgen vier grote delen die we hieronder kort toelichten.
%\textit{Deel I} bevat nuttige achtergrondinformatie over zwarte gaten, de twee onderzoeksgebieden die hierboven werden geschetst komen aan bod in \textit{Deel II} en \textit{Deel III}. \textit{Deel IV} tenslotte bevat een conclusie en een aantal appendices.

\subsubsection{Deel I: Achtergrondinformatie over zwarte gaten}
In dit deel wordt in een wiskundige taal nuttige achtergrond geschetst i.v.m.~zwarte gaten en snaartheorie. Het is gericht op fysici die geen technische kennis hebben van de snaartheorie, maar wel een idee hebben van Einsteins relativiteitstheorie.

\begin{itemize}
\item[\ra]\emph{\underline{Hoofdstuk \ref{c:BH_Playground}}} legt uit wat een zwart gat is in relativiteitstheorie en behandelt
%Het concept van een zwart gat dat een lading draagt komt ook aan bod. 
in detail de entropie, de thermische straling van een zwart gat en de geas\-so\-ci\-eer\-de problemen (informatieparadox, geen microscopisch begrip van entropie).
\item[\ra]\emph{\underline{Hoofdstuk \ref{c:IS}}} biedt een idee hoe zwarte gaten te construeren zijn als oplossingen van snaartheorie. De nadruk ligt op de limiet waarin de snaren zich gedragen als puntdeeltjes. In dit regime is de theorie goed benaderd door supergravitatie. In het bijzonder wordt getoond hoe de entropie van supersymmetrische zwarte gaten wordt verklaard door snaartheorie.
%, door het zwart gat te zien als een constructie van D-branen. Als laatste schijnen we een licht op wat het verschil is tussen supersymmetrische en niet-supersymmetrische zwarte gaten.
\end{itemize}



\subsubsection{Deel II: Vereenvoudigde beschrijving van niet-supersymmetrische zwarte gaten}
%Om het onderzoek van dit deel te kaderen, moeten we even wat wiskundig kader schetsen. 
Dit deel behandelt zwarte gaten in supergravitatie, meer bepaald op de structuur van de bewegingsvergelijkingen voor zwarte-gatoplossingen. De su\-per\-gra\-vi\-tatie-beschrijving is een uitbreiding van Einsteins relativiteitstheorie en daarom bevat ze net als Einsteins theorie een metriek die de kromming van de ruimte-tijd beschrijft. Daarnaast komen er nog vele andere deeltjes aan bod, die in technische termen vectorvelden en scalaire velden genoemd worden. Vooral de scalaire velden zijn belangrijk, omdat ze in de algemene relativiteitstheorie niet voorkomen. Voor supersymmetrische oplossingen zijn de bewegingsvergelijkingen van deze velden eerste-orde differentiaalvergelijkingen, terwijl voor een algemene niet-supersymmetrische oplossing dit normaal gekoppelde differentiaalvergelijkingen zijn van tweede orde. In dit deel tonen we aan dat die idee fout is: er zit meer structuur in de bewegingsvergelijkingen van niet-supersymmetrische oplossingen zit dan aangenomen wordt (ze zijn vaak eerste-orde).

\begin{itemize}
\item[\ra]\emph{\underline{Hoofdstuk \ref{c:BJ}}} %Begint met een overzicht van eerste orde formalismes in de literatuur, i.h.b.~voor supersymmetrische zwarte gaten en hun eerste-orde vergelijkingen. 
bouwt voort op resultaten van \cite{Miller:2006ay} en bespreekt ons werk \cite{Janssen:2007rc} waarin we tonen dat voor eenvoudige zwarte gaten in supergravitatie met \'e\'en scalair veld, de bewegingsvergelijkingen altijd van eerste orde zijn, ook voor niet-supersymmetrische oplossingen. Het resultaat is ook van toepassing op zogenaamde zwarte $p$-branen, analogen van zwarte gaten die zich uitstrekken in $p$ dimensies.
\item[\ra]\emph{\underline{Hoofdstuk \ref{c:JP-Gradient_Flow}}} bespreekt in detail de voorwaarden waaraan een gecombineerd systeem van gravitatie, vectoren en scalaire velden moet voldoen opdat de bewegingsvergelijkingen voor niet-supersymmetrische zwarte gaten kunnen geschreven worden als eerste-orde vergelijkingen die dezelfde vorm hebben als de vergelijkingen voor supersymmetrische zwarte gaten. Door de eis van sferische symmetrie, zijn de vectorvelden automatisch bepaald en is het voldoende een effectieve actie voor de scalaire velden en \'e\'en functie uit de metriek te bekijken. Voor supersymmetrische oplossingen zijn de bewegingsvergelijkingen van de scalairen en de metriekfunctie eerste-orde vergelijkingen, die bovendien volledig bepaald zijn door de gradi\"ent van \'e\'en functie, de \emph{superpotentiaal} genoemd. De voorwaarde opdat de eerste-orde vergelijkingen voor niet-supersymmetrische oplossingen van dezelfde vorm zijn is dat de effectieve actie een Liouville integreerbaar systeem beschrijft. Liouville integreerbaarheid wil zeggen dat er voor $n$ scalairen en metriekfuncties in totaal $n$ constanten van de beweging zijn, die commuteren onder de standaard Poisson haken. Dit hoofdstuk behandelt ons werk \cite{Perz:2008kh} in die context en geeft een aantal voorbeelden om de formele idee\"en te staven.
\end{itemize}
%\comment{LINKS NAAR EIGEN WERK}

\subsubsection{Deel III: Microscopische structuur van supersymmetrische zwarte gaten}
Dit deel wil een interpretatie geven van de microtoestanden van zwarte gaten in het realistische geval van drie ruimtelijke dimensies. Het blijkt dat er in de gravitatietheorie\"en die volgen uit de snaartheorie (supergravitatie, zie eerder), ook stabiele configuraties zijn van verschillende zwarte gaten die op vaste afstanden aan mekaar gebonden zijn. We noemen deze multi-center zwarte gaten. Multi-center zwarte gaten ontstaan als de gravitationele aantrekking en de afstoting door de elektrische lading die ze dragen mekaar exact opheffen. Deze multi-center gaten blijken een grote rol te spelen in de interpretatie van microtoestanden van zwarte gaten, daarom dat ze hier aan bod komen.
\begin{itemize}
\item[\ra]\emph{\underline{Hoofdstuk \ref{c:FB}}} bevat een overzicht van het pluisbal (Eng.~fuzzball) idee.
\item[\ra]\emph{\underline{Hoofdstuk \ref{c:JR}}} maakt de link tussen bepaalde pluisbal oplossingen in vier ruimtelijke dimensies en multi-center zwarte gaten in drie ruimtelijke dimensies. Dit toont aan dat we microtoestanden van bepaalde zwarte gaten kunnen zien als multi-center configuraties.
\item[\ra]\emph{\underline{Hoofdstuk \ref{c:TL}}} is een eerste poging om een duidelijke interpretatie te geven van de microtoestanden van een algemeen supersymmetrisch zwart gat in termen van multi-center configuraties. De entropie en de oorsprong van de microtoestanden konden niet verklaard worden, maar er werd wel een zeer interessante manier gevonden om de G\"odel-ruimte (zie onder) te vinden als een supersymmetrische oplossing van snaartheorie.
\item[\ra]\emph{\underline{Hoofdstuk \ref{c:GB}}} De G\"odel-ruimte uit het vorige hoofdstuk heeft een aantal prob\-le\-men: deze ruimte is een soort `tijdmachine', het is mogelijk om door te tijd te reizen in de G\"odel-ruimte. Ruimtes met die eigenschap leiden tot nare gevolgen\footnote{Zoals de grootvader paradox, zie bv.~\href{http://en.wikipedia.org/wiki/Grandfather_paradox}{\texttt{http://en.wikipedia.org/wiki/Grandfather\_paradox}}.}, waardoor Stephen Hawking voorstelde dat ze niet kunnen ontstaan in fysische processen in zijn `chronologie-beschermingshypothese'. We on\-der\-zoch\-ten een manier om op natuurlijke wijze die chronologiebescherming te realiseren. In een vereenvoudigde opstelling slaagden we erin. Door gebruik te maken van de AdS/CFT correspondentie\footnote{Die relateert een bepaalde geometrie (AdS) aan een bepaalde kwantumveldentheorie (CFT)}, konden we aantonen dat omwille van kwantummechanische principes de regio in de G\"odel-ruimte waar een tijdmachine kan ontstaan niet gevormd wordt.
\end{itemize}
\subsubsection{Deel IV: Conclusie en appendix}
\begin{itemize}
\item[\ra]\emph{\underline{Hoofdstuk \ref{c:Conclusions}}} bevat een besluit bij het onderzoek in dit werk.
\item[\ra]\emph{\underline{Appendices:}} %in appendix \ref{c:Intro_SUGRA} wordt wat achtergrond geschetst van supergravitatie, 
Appendix \ref{app:SS} geeft wat technische achtergrond i.v.m.~een dimensionele reductie uit hoofdstuk \ref{c:JP-Gradient_Flow} en een oplossingsmethode van hoofdstuk \ref{c:TL}. Appendix \ref{app:NDL} tenslotte is deze Nederlandse samenvatting.
\end{itemize}
\selectlanguage{english}

==> DankwoordLight.tex <==
\chapter*{Woord van dank}
\addcontentsline{toc}{chapter}{Acknowledgments}
\setlength{\parindent}{5mm}
% Vier jaar (of toch bijna) liggen er tussen het voltooien van dit werk en mijn aantreden als doctoraatstudent op ``het zesde verdiep'', de hoogste gang van het natuurkundegebouw in de campus in Heverlee, de verdieping waar de theoretische fysica is gehuisvest. In die vier jaar kruisten er veel mensen mijn pad, die ik van harte zou willen bedanken. In de eerste plaats zijn dat mijn promotor, Toine, en mijn lieve \emph{keppeke} Evelien. Zonder hen hadden mijn leven en doctoraatswerk de afgelopen 4 jaar er behoorlijk anders en ongetwijfeld armer uitgezien.

% E\'en september 2006, een maand voor aanvang van mijn doctoraat. Het is warm, zeer warm. De zomer laat haar tanden nog eens zien. Ik heb afspraak bij Toine op het bureau. Hij zit tegenover me, in korte broek en T-shirt, de racefiets waarmee hij naar het werk reed leunt tegen zijn uitpuilende archiefkast. Terwijl hij even nadenkt over mijn vraag of ik bepaalde interessante wiskunde niet meer mag bestuderen in het kader van mijn doctoraat, kijk ik wat rond. Ik zie de stapels papier, de boeken, de kast vol documenten. Op dat moment kan ik me helemaal niet inbeelden dat ik vier jaar later een gelijkaardig papierimperium zal hebben opgebouwd. Toine haalt me uit mijn dromerigheid met een antwoord dat to the point is: ``Het heeft geen zin om veel dingen te studeren, als je ze later niet zal gebruiken. Maak je enkel meester van wat je nodig zal hebben, de rest vergeet je toch''. In hetzelfde gesprek zet Toine me ook op de rails voor mijn eerste project, waarmee ik een maand later officieel mijn doctoraat zal beginnen. Die woorden van mijn promotor heb ik toegepast op dat eerste project (een klein jaar later mijn eerste artikel) en op mijn hele doctoraat. Ze drukken perfect de manier uit waarop ik steun kreeg van mijn promotor: af en toe een paar tips, veel vrijheid, zolang het ergens toe leidt. Dank, Toine, voor de begeleiding-vanop-afstand, de mogelijkheden om mijn eigen weg te zoeken en de gidsende hand tussendoor. Misschien nog wel het meest bedankt voor die initi\"ele raad, die meteen de toon zette voor mijn onderzoek.

% Dit werk is er maar gekomen dankzij de hulp van vele mensen.  Daarom zou ik graag hen die het verschil maakten willen bedanken. 

% ``Het heeft geen zin om veel dingen te studeren, als je ze later niet zal gebruiken. Maak je enkel meester van wat je nodig zal hebben, de rest vergeet je toch''. Deze raad die mijn promotor  Antoine Van Proeyen vier jaar geleden gaf, heb ik toegepast op mijn hele doctoraat. Ze drukken perfect de manier uit waarop je mij steunde, Toine: regelmatige tips, veel vrijheid, zolang het ergens toe leidt. Dank je voor de begeleiding-vanop-afstand, de mogelijkheden om mijn eigen weg te zoeken, de gidsende hand tussendoor, het openen van buitenlandse deuren en om heel deze thesis zo nauwgezet door te nemen en bij te sturen waar nodig.\\\indent
% Bram W. voor de grote interesse en hulpvaardigheid met het op punt stellen van de introducerende stukken (en het onverbloemd aanduiden van t\'e technische delen), en samen met Eliran bedankt voor de kans om mijn vakgebied in bevattelijke(re) termen proberen uit te leggen. Dank Toine, natuurlijk, om alles zo nauwgezet door te nemen en in detail suggesties te formuleren. Evelien, je hebt ook behoorlijk wat mogen ondergaan qua uitleg en vragen, nalezen en beluisteren van mijn steeds wijzigende plannen voor de structuur. Dank je voor je hulp. 
% Graag wil ik ook nadrukkelijk de andere leden danken van mijn examenjury, namelijk Walter Troost, Okki Indekeu, D\'esir\'e Boll\'e aan de K.U.Leuven, and thank you Jos\'e Figueroa-O'Farrill and Iosif Bena, for finding the time to read and assess my doctoral work and come to Leuven for the defense. Daarbuiten ook \emph{special thanks to} Krist Maes voor de interesse, Frans Cerulus voor het aanwijzen van de nijpende typfouten, Enrico Carlon voor de in-house seminars en de andere stafleden voor de aangename contacten. In het bijzonder denk ik aan Jos Rogiers voor de drie jaren van goede samenwerking bij de lessenreeksen en Walter Troost voor alle tips, discussies over didactiek en lesmethodes, het aangename contact in de lessen electrodynamica, de begeleiding bij studentenprojecten en heel veel kleine momenten van feedback. Dankjewel ook Anita, Christine en Bavo en de laatste jaren Anneleen en Filip voor ondersteuning, vooral Filip om zover buiten de lijntjes te kleuren en een pak meer te doen dan wat de jobomschrijving zegt. Dank aan de Belgische belastingbetaler, die via een aspirant-beurs van het Fonds voor Wetenschappelijk Onderzoek dit doctoraatsproject heeft mogelijk gemaakt.\\\indent

First of all, thank you Toine, my supervisor, for your advice, your guiding hand, the chances of growing in the field. Thanks also to the members of the jury, Walter Troost, Okki Indekeu, D\'esir\'e Boll\'e at K.U.Leuven and thank you Jos\'e Figueroa-O'Farrill and Iosif Bena, for finding the time to read and assess my doctoral work and come to Leuven for the defense. 

% \footnote{Deze investering lijkt voor sommigen misschien niet de moeite waard -- waarom geld pompen in een abstracte ver-van-mijn-bed-show als snaartheorie en aanverwanten? -- maar is in mijn ogen uiterst belangrijk. Wanneer we fundamenteel onderzoek (van allerlei aard) niet meer steunen, zagen we de poten weg waarop onze maatschappij gestoeld is.}
Thank you, my collaborators, for many discussions and for shaping this work: thank you 
Bert, Jan, Paul, Thomas (times three: Thomas, Tokke and Tommy),  Dieter, Joris,  Walter, Jos\'e and Toine
% Bert Janssen, Jan Perz, Paul Smyth, Thomas Van Riet, Thomas Wyder, Tommy Levi, Dieter Van den Bleeken, Joris Raeymaekers, Jos\'e Miguel Figueroa-O'Farrill, Toine Van Proeyen, Walter Van Herck 
(and also Frederik, Bram G., Fran\c cois, Jan D., Eric, Oscar, Andr\`es and Wieland for numerous discussions and work ``behind the scenes''). 
% Een aantal mensen van wie ik veel leerde, zou ik speciaal willen bedanken. 

Finally, this work was supported by an Aspirant fellowship of the FWO-Vlaanderen during the 4 PhD years, and in part by the European Community’s Human Potential Programme under contract MRTN-CT-2004-005104 ‘Constituents, fundamental forces and symmetries of the universe’, by the Federal Office for Scientific, Technical and Cultural Affairs through the ‘Interuniversity Attraction Poles Programme – Belgian Science Policy’ P6/11- P, and in part by the FWO - Vlaanderen, project G.0235.05.   


{\it Note: for those looking for a thank you to all who contributed outside the work environment, see the printed version.}

{}\raggedleft Bert Vercnocke,\\
\raggedleft juli 2010

==> preamble_bert_thesis2.tex <==

\usepackage{slashed}
%\documentclass[JHEP3,twoside,12pt]{report}
%\documentclass[fleqn,11pt,twoside]{report}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%xfig necessities
\renewcommand\baselinestretch{1.0}           % single space
\usepackage{color}		% Need the color package
\usepackage{epsfig}
%accents/umlaurs... on letters (\diaeresis{i})
\usepackage{metre}

\usepackage{curves}
% for ticks (checkmarks) and X's; right/left hands
\usepackage{bbding}
% for special arrows
\usepackage{pifont}
%for subfigures (side-by-side}
\usepackage{subfigure}
%small captions
\usepackage[small]{caption}
% Different font in captions
\newcommand{\captionfonts}{\small \em}
\newcommand{\sectionfonts}{\small \sffamilly}
%cool itemizes
%\usepackage{mathabx}
%\usepackage{wasysym}
%\usepackage{MnSymbol}

\usepackage{multirow}

\makeatletter  % Allow the use of @ in command names
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{{\captionfonts #1: #2}}%
  \ifdim \wd\@tempboxa >\hsize
    {\captionfonts #1: #2\par}
  \else
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
\makeatother 

\usepackage{fancyhdr}
%\usepackage[dvips]{graphicx}
%\usepackage{graphpap}
%\usepackage{ifthen}
\usepackage{enumerate}
%\usepackage{cite}
%\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{calrsfs}
\usepackage[mathscr]{eucal}
\usepackage[errorshow]{tracefnt}
\usepackage{makeidx}
%\usepackage{fancybox}\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{array}
\usepackage{amsthm}
\usepackage{eucal}
\usepackage{setspace}
\usepackage{tikz}

% \newcommand{\mymk}[1]{%
%   \tikz \node[anchor=south west, draw,circle, inner sep=0pt, minimum size=4mm,
%     text height=2mm]{\ensuremath{#1}} ;}
% \newcommand{\vm}{\mymk{v}}
% \newcommand{\sm}{\mymk{s}}
%\usepackage{eufrak}
\usepackage{epsfig}
%\usepackage{epstopdf}
\usepackage{pgf}
% \usepackage{slashed}
% \usepackage{makeidx}
%\usepackage[apple mac]{inputenc}
%\usepackage[french]{babel}
%\usepackage{picins}
%\usepackage{showkeys}

%Change fonts
%\usepackage[T1]{fontenc}
%\usepackage[light,condensed,math]{kurier}
%% \usepackage[T1]{fontenc}
% \usepackage[adobe-utopia]{mathdesign}
%
% \usepackage[T1]{fontenc}
% \usepackage{fourier} %%% I had this before
%
% \usepackage[T1]{fontenc}
% \usepackage{mathptmx}
%
% \usepackage[T1]{fontenc}
% \usepackage[sc]{mathpazo}
% \linespread{1.05}
%
% \usepackage[T1]{fontenc}
% \usepackage{efont,mathesf}
% \renewcommand*\oldstylenums[1]{{\fontfamily{esfod}\selectfont#1}}
%
% \usepackage[T1]{fontenc}
% \usepackage{fouriernc}

%Fancy pancy commands (definitions, theorems, anything really)
%
% Outlook/reorientation
\newcommand{\outlook}[2]
{
%\hrule
%\vspace{}
\begin{itemize}
  \item[\rh] \underline{\emph{#1}} #2
\end{itemize}
%\vspace{}
%\hrule
}
%
% Punchline (``Abstract'' of each chapter)
\newcommand{\punchlineOLD}[1]
{
\begin{center}
\framebox{\hspace{.5cm}\parbox{11cm}{\vspace{.3cm}{{\centering \Large \it  Summary:\vspace{.3cm}\\}{\footnotesize
 #1}}\vspace{.3cm}}\hspace{.5cm}}
\end{center}
}
%%% Nieuwe versie, nu in gebruik:
\newcommand{\punchline}[1]
{
\begin{center}
% \framebox{
% \hspace{.5cm}
\parbox{11cm}{\vspace{.3cm}{{\sectiontypeset\selectfont Summary{\hrule}\vspace{.3cm}}{\footnotesize \it
 #1}}\vspace{.3cm}}
% \hspace{.5cm}
% }
\end{center}
}
%%% In het Nederlands:
\newcommand{\ponslijn}[1]
{
\begin{center}
% \framebox{
% \hspace{.5cm}
\parbox{11cm}{\vspace{.3cm}{{\sectiontypeset\selectfont Samenvatting{\hrule}\vspace{.3cm}}{\footnotesize \it
 #1}}\vspace{.3cm}}
% \hspace{.5cm}
% }
\end{center}
}
%
% Outline (``Outline'' of next chapter/section...)
\newcommand{\outline}[1]
{
\subsubsection{Outline}
{#1}
}
%

%Definitions
\def\symB{\hspace{.2cm}$\bullet$\hspace{.3cm}}
\def\RN{Reissner-Nordstr\"om }
\newcommand{\rf}[1]{(\ref{#1})}
\def\C{{C}}

\def\B{{B}}

%Group theory
\def\unit{\hbox{$1\hskip -1.2pt\vrule depth 0pt height 1.6ex width 0.7pt
\vrule depth 0pt height 0.3pt width 0.12em$}}
\newcommand{\E}{\mathop{\rm E}}
\newcommand{\SU}{\mathop{\rm SU}}
\newcommand{\SO}{\mathop{\rm SO}}
\newcommand{\bO}{\mathop{\rm {}O}}
\newcommand{\CSO}{\mathop{\rm CSO}}
\newcommand{\ISO}{\mathop{\rm ISO}}
\newcommand{\U}{\mathop{\rm {}U}}
\newcommand{\USp}{\mathop{\rm {}USp}}
\newcommand{\Sp}{\mathop{\rm {}Sp}}
\newcommand{\OSp}{\mathop{\rm {}OSp}}
\newcommand{\Symp}{\mathop{\rm {}Sp}}
\newcommand{\Sl}{\mathop{\rm {}S}\ell }
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\Tr}{Tr}

%comments etc.
%
%Plain comments
\newcommand{\comment}[1]{[$\clubsuit${\ {\bf #1}}]}
%Questions of whether to leave out text/put it in for Toine
% \newcommand{\tokeep}[1]{[{XXX \bf #1 XXX}]}
\newcommand{\Bil}[2]{\bar {#1} #2}




%Common phrases
\def\ansatz{{Ansatz}}
\def\ansatze{{Ans\"atze}}
\def\worldvolume{{world volume{}}}
\def\spacetime{{space-time{}}}
\def\spacetimes{{space-times{}}}
\def\worldvolumes{{world volumes{}}}
\def\worldline{{world line{}}}
\newcommand{\AdS}[1]{{\rm AdS}_{#1}}
\newcommand{\CY}[1]{{\rm CY}_{#1}}
\newcommand{\sS}[1]{{\rm S}^{#1}}

%Technical commands
\renewcommand{\d}{\textrm{d}}
\newcommand{\ft}[2]{{\textstyle\frac{#1}{#2}}}
\newcommand{\Hodge}{\mathop{\star}}
\newcommand{\Real}{\mathbb{R}}
% D anti-branes
\newcommand{\Db}[1]{\overline{D}#1}

%Special Characters
\def\e{{\mathrm e}}
\def\eps{{\epsilon}}
\def\veps{{\varepsilon}}
\def\rme{{\rm e}}
\def\rmi{{\rm i}}
\def\rmd{{\rm d}}
\def\Re{\mathop{\rm Re}\nolimits}
\def\Im{\mathop{\rm Im}\nolimits}

%specific to JP article
\newcommand{\de}{\textrm{d}}

%specific to proceedings
\newcommand{\SL}{\mathop{\mathrm{SL}}}
\newcommand{\GL}{\mathop{\mathrm{GL}}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\QE}{q_e}%{Q_\mathrm{e}}
\newcommand{\QM}{q_m}%{Q_\mathrm{m}}
\newcommand{\QT}{Q_\mathrm{T}}
\newcommand{\Qc}{{\cal Q}}
\newcommand{\qE}{q_\mathrm{e}}
\newcommand{\qM}{q_\mathrm{m}}
\newcommand{\JE}{j_\mathrm{e}}
\newcommand{\JM}{j_\mathrm{m}}
\newcommand{\abs}[1]{\lvert #1\rvert}
\newcommand{\im}{\mathrm{i}}

%Arrows and other alternative item symbols
\newcommand{\ra}{\ding{242}}
\newcommand{\rh}{\HandRight}
\newcommand{\rhb}{\HandCuffRight}
\newcommand{\rab}{{\ArrowBoldDownRight}}
\newcommand{\todo}{\ding{42}}
%
\newcommand{\tickb}{\ding{52}}
\newcommand{\tick}{\Checkmark{}}

%Calligraphic symbols
\def\ca{{\cal{A}}}
\def\cb{{\cal{B}}}
\def\cf{{\cal{F}}}
\def\cg{{\cal{G}}}
\def\cq{{\cal{Q}}}
\def\ch{{\cal{H}}}
\def\ce{{\cal{E}}}
\def\ci{{\cal{I}}}
\def\cl{{\cal{L}}}
\def\cm{{\cal{M}}}
\def\cn{{\cal{N}}}
\def\Cn{{\cal{N}}}
\def\co{{\cal{O}}}
\def\ck{{\cal{K}}}
\def\cw{{\cal{W}}}
\def\cv{{\cal{V}}}
\def\cc{{\cal C}}
\def\Mg{{\cal M}}
%epsilons etc.
\def\eps{{\epsilon}}
\def\vareps{{\varepsilon}}

%Convention in normalization el. charge and Hamilonian energy 
\def\Conv{{\gamma}}
\def\En{{E}}
%index etc.
\newcommand{\imp}[1]{{\it \hyperpage{#1}}}
\newcommand{\defn}[1]{{\bf \hyperpage{#1}}}
\newcommand{\fn}[1]{#1n} %(something in footnote)

\makeindex

%Commando's voor parti\"ele e \item Gradi\"ent flown totala afgeleiden:
%-----parti\"ele----afgeleide-----------------------------------------------------------
\newcommand{\pf}[2]{\frac{\partial {#1} }{\partial {#2}}}
%-----totale--------afgeleide-----------------------------------------------------------
\newcommand{\ta}[2]{\frac{\de {#1} }{\de {#2}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Specific for symmetric spaces appendix
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bSL}{\mathop{\rm SL}}
\newcommand{\bGL}{\mathop{\rm GL}}
\newcommand{\Gl}{\mathop{\rm {}G}\ell }
\newcommand{\Spin}{\mathop{\rm {}Spin}}
\newcommand{\CK}[2]{\langle {#1},{#2}\rangle}
\newcommand{\f}[3]{f_{#1#2}{}^{#3}}
\newcommand{\df}{\equiv}
\newcommand{\vc}{\overrightarrow}
\newcommand{\Ea}{E_{\vec \alpha}}
\newcommand{\Eb}{E_{\vec \beta}}
\newcommand{\bSLn}[2]{\bSL({#1},\mathbb{#2})}
\newcommand{\bGLn}[2]{\bGL({#1},\mathbb{#2})}
\newcommand{\bsl}[2]{\mathfrak{sl}({#1},\mathbb{#2})}
\newcommand{\bgl}[2]{\mathfrak{gl}({#1},\mathbb{#2})}
\newcommand{\bgln}[2]{\mathfrak{gl}({#1},\mathbb{#2})}
\newcommand{\bsln}[2]{\mathfrak{sl}({#1},\mathbb{#2})}
\newcommand{\bU}{\mathop{\rm {}U}}
\newcommand{\bSU}{\mathop{\rm {}SU}}
\newcommand{\bso}{\mathfrak{so}}
\newcommand{\bsu}{\mathfrak{su}}
\newcommand{\bu}{\mathfrak{u}}
\newcommand{\bo}{\mathfrak{o}}
\newcommand{\bsun}[1]{\mathfrak{su}({#1})}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\diag}{{	\rm diag}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% for exercices:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{exercise}[section]
\renewcommand{\theexercise}{\thesection.\arabic{exercise}}
\newcommand{\bexer}{
   \begin{list}{\bf Exercise \theexercise : }{\refstepcounter{exercise}
           \setlength {\rightmargin}{\leftmargin}}\item }
\newcommand{\eexer}{\end{list}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% for examples:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{example}[section]
\renewcommand{\theexample}{\thesection.\arabic{example}}
\newcommand{\bexam}{
   \begin{list} {\noindent \emph{Example \theexample: }}{\refstepcounter{example}
           \setlength {\rightmargin}{\leftmargin}}\item }
\newcommand{\eexam}{\end{list}}

% Define pagestyle
% \pagestyle{fancy}
% \fancyhf{}
% \renewcommand{\chaptermark}[1]{\markboth{ \emph{#1}}{}}
% \fancyhead[LO]{}
% \fancyhead[RE]{\leftmark}
% \fancyfoot[LE,RO]{\thepage}

\RequirePackage{hyperref}

\numberwithin{equation}{section}

%change the index to three columns
\usepackage{multicol}
\makeatletter
%smaller letters
\renewcommand\@idxitem{\footnotesize\par\hangindent 20\p@}
\renewcommand\subitem{\@idxitem \hspace*{10\p@}}
\renewcommand\subsubitem{\@idxitem \hspace*{15\p@}}
\renewcommand\indexspace{\par \vskip 15\p@ \@plus2\p@ \@minus1.5\p@\relax}
%rest
\renewenvironment{theindex}
  {\if@twocolumn
      \@restonecolfalse
   \else
      \@restonecoltrue
   \fi
   \setlength{\columnseprule}{0pt}
   \setlength{\columnsep}{35pt}
   \begin{multicols}{3}[\section*{\indexname}]
   \markboth{\MakeUppercase\indexname}%
            {\MakeUppercase\indexname}%
   \thispagestyle{plain}
   \setlength{\parindent}{0pt}
   \setlength{\parskip}{0pt plus 0.3pt}
   \relax
   \let\item\@idxitem}%
  {\end{multicols}\if@restonecol\onecolumn\elseclearpage\fi}
\makeatother

%appendix per chapter
\usepackage{appendix}

%table notes
\usepackage{threeparttable}
\usepackage{ctable2}


%wrapping figures
\usepackage{wrapfig}

%page adjustments
 \addtolength{\textwidth}{1mm}
 \addtolength{\textheight}{.6cm}
 \addtolength{\hoffset}{0.5mm}
%  \addtolength{\voffset}{-1.5cm}



% \usepackage{lettrine}
%for chapter styles
%\usepackage{fncychap}

%For quotes
% \renewcommand\chapterheadstartvskip{\vspace*{-5\baselineskip}}


==> preamble_phd_template2.tex <==
\usepackage[square,comma]{natbib}

% \RequirePackage[calcwidth]{titlesec}
% 
% \titleformat{\section}[hang]{\sffamily\bfseries}
% {\Large\thesection}{12pt}{\Large}[{\titlerule[0.5pt]}]

\bibpunct{[}{]}{,}{n}{}{;}
\usepackage{graphicx}
\usepackage[english,dutch]{babel}
\usepackage[ps2pdf,bookmarks,breaklinks,pdfborder={0 0 0}]{hyperref}




\usepackage{placeins} % provides \FloatBarrier command
\usepackage{color}
\usepackage{booktabs}
\usepackage{textcomp} % nice greek alphabet
\usepackage{pifont}   % Dingbats
%\usepackage[showboxes]{textpos}
\usepackage{textpos}
\usepackage{subfigure}
% TEXTPOS options
\definecolor{gray}{rgb}{0.600,0.600,0.600}

\setlength{\TPHorizModule}{1mm}
\setlength{\TPVertModule}{1mm}

% FONTS
% \usepackage{microtype}
% \usepackage[T1]{fontenc}
% \usepackage{lmodern}
% \newcommand{\labfont}{\fontfamily{phv}\selectfont} % fonts used in labels
% \usepackage{sectsty}
% \allsectionsfont{\usefont{OT1}{phv}{bc}{n}}
% \DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

% FONTS
\usepackage{microtype}
%\usepackage[T1]{fontenc}
\usepackage{lmodern}
\newcommand{\labfont}{\fontfamily{phv}\selectfont} % fonts used in labels
\usepackage{sectsty}
\allsectionsfont{\sectiontypeset\selectfont}%{\sectiontypeset\bfseries\selectfont}
\partfont{\sffamily\fontsize{32}{50}\selectfont}

% \allchaptersfont{\sffamily}
\newcommand{\chaptertypeset}{\sectiontypeset\selectfont}%{\sectiontypeset\bfseries\selectfont}
\newcommand{\sectiontypeset}{\sffamily}%{\fontfamily{ptm}}%{\fontfamily{phv}}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\usepackage[times]{quotchap_Bert}
% \usepackage{mathptmx}
%  \usepackage{helvetica+m}
% \fontfamily{ptm}

% % FONTS
% \usepackage{microtype}
% \usepackage[T1]{fontenc}
% \usepackage{lmodern}
% \newcommand{\labfont}{\fontfamily{phv}\selectfont} % fonts used in labels
% \usepackage{sectsty}
% \allsectionsfont{\sffamily}
% \DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

% % TABLE OF CONTENTS
\usepackage[titles]{tocloft}
\renewcommand{\cftpartfont}{\large\sectiontypeset\bfseries\selectfont}
\renewcommand{\cftchapfont}{\sectiontypeset\bfseries\selectfont}
\renewcommand{\cftchappagefont}{\sectiontypeset\bfseries\selectfont}
\setlength{\cftbeforechapskip}{-0.05ex}
\setlength{\cftbeforesecskip}{-1.5ex}
\setlength{\cftbeforesubsecskip}{-1.5ex}
% \renewcommand{\@dotsep}{10000}


%% Control the fonts and formatting used in the table of contents.

%% Aesthetic spacing redefines that look nicer to me than the defaults.
% \setlength{\cftbeforechapskip}{2ex}
% \setlength{\cftbeforesecskip}{0.5ex}
% Use Helvetica-Narrow Bold for Chapter entries
% \renewcommand{\cftchapfont}{\fontsize{11}{13}\usefont{OT1}{phv}{bc}{n}\selectfont}
% \renewcommand{\cftchappagefont}{\usefont{OT1}{phv}{bc}{n}\selectfont}


% 
% PAGE LAYOUT
% \setlength{\textwidth}{16truecm}
% \setlength{\textheight}{22.0truecm} %\pagestyle{plain}
% \setlength{\evensidemargin}{.25truecm}
% \setlength{\oddsidemargin}{.25truecm}
% \setlength{\jot}{10pt}
% \setlength{\parindent}{0mm}
% \setlength{\parskip}{7.2pt}
% \raggedbottom

% PAGE CONTROL AND QUOTATION
\def\startchapter{
  \ifodd\count0
    \clearpage\thispagestyle{myheadings}\vspace*{\fill}\clearpage
  \else
    \vspace*{\fill}\clearpage\fi}


% 
%% CLEARDOUBLEPAGE
\makeatletter
\def\cleardoublepage{\clearpage\if@twoside \ifodd\c@page\else%
\hbox{}%
\thispagestyle{empty}%
\newpage%
\if@twocolumn\hbox{}\newpage\fi\fi\fi}
\makeatother

% FIGURES
\renewcommand{\topfraction}{1}  % max fraction of floats at top
\renewcommand{\bottomfraction}{1} % max fraction of floats at bottom
% Parameters for TEXT pages (not float pages):
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}     % 2 may work better
\setcounter{dbltopnumber}{2}    % for 2-column pages
\renewcommand{\dbltopfraction}{0.9} % fit big float above 2-col. text
\renewcommand{\textfraction}{0.07}  % allow minimal text w. figs
% Parameters for FLOAT pages (not text pages):
\renewcommand{\floatpagefraction}{0.7}  % require fuller float pages
% N.B.: floatpagefraction MUST be less than topfraction !!
%\renewcommand{\dblfloatpagefraction}{0.7} % require fuller float pages

% CLAP
\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathrlap{\mathpalette\mathrlapinternal}
\def\mathclap{\mathpalette\mathclapinternal}
\def\mathllapinternal#1#2{\llap{$\mathsurround=0pt#1{#2}$}}
\def\mathrlapinternal#1#2{\rlap{$\mathsurround=0pt#1{#2}$}}
\def\mathclapinternal#1#2{\clap{$\mathsurround=0pt#1{#2}$}}

%CPV
% \def\Xint#1{\mathchoice
% {\XXint\displaystyle\textstyle{#1}}%
% {\XXint\textstyle\scriptstyle{#1}}%
% {\XXint\scriptstyle\scriptscriptstyle{#1}}%
% {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
% \!\int}
% \def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
% \vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
% \def\ddashint{\Xint=}
% \def\dashint{\Xint-}

% VEC
\def\vecc#1{{\bf\bm{#1}}}

% DTILDE
\def\dtilde#1{\mathrlap{\rlap{\raise1.2pt\hbox{$\mathsurround=0pt%
\tilde{\phantom{\hbox{$#1$}}}$}}\tilde{\phantom{\hbox{$#1$}}}}#1}

% UBAR
\def\ubar#1{\mathrlap{\rlap{\hbox{$\mbox{\rule{-0.1pt}{0pt}%
                    \mathsurround=0pt\b{\phantom{\hbox{$#1$}}}}$}}}{#1}}

% ORPHANS AND WIDOWS
\clubpenalty=9999
\widowpenalty=9999

% HYPHENATION
\hyphenpenalty=5000
\tolerance=1500
% 
% 
% 
% \usepackage{titlesec}
% \titleformat{\section}[hang]{\sffamily\bfseries}
% {\Large\thesection}{12pt}{\Large}[{\titlerule[0.5pt]}]
